PassGoodPool: Joint Passengers and Goods Fleet Management with Reinforcement Learning aided Pricing, Matching, and Route Planning

The ubiquitous growth of mobility-on-demand services for passenger and goods delivery has brought various challenges and opportunities within the realm of transportation systems. As a result, intelligent transportation systems are being developed to maximize operational profitability, user convenience, and environmental sustainability. The growth of last mile deliveries alongside ridesharing calls for an efficient and cohesive system that transports both passengers and goods. Existing methods address this using static routing methods considering neither the demands of requests nor the transfer of goods between vehicles during route planning. In this paper, we present a dynamic and demand aware fleet management framework for combined goods and passenger transportation that is capable of (1) Involving both passengers and drivers in the decision-making process by allowing drivers to negotiate to a mutually suitable price, and passengers to accept/reject, (2) Matching of goods to vehicles, and the multi-hop transfer of goods, (3) Dynamically generating optimal routes for each vehicle considering demand along their paths, based on the insertion cost which then determines the matching, (4) Dispatching idle vehicles to areas of anticipated high passenger and goods demand using Deep Reinforcement Learning (RL), (5) Allowing for distributed inference at each vehicle while collectively optimizing fleet objectives. Our proposed model is deployable independently within each vehicle as this minimizes computational costs associated with the growth of distributed systems and democratizes decision-making to each individual. Simulations on a variety of vehicle types, goods, and passenger utility functions show the effectiveness of our approach as compared to other methods that do not consider combined load transportation or dynamic multi-hop route planning.

==> DARM.tex <==
\section{DARM Distributed Optimization Phase:}
As shown earlier, there is no polynomial time algorithm that achieves an optimal solution for our demand-aware route planning problem. However, several studies show that Insertion is an effective approach to greedily deal with the shared mobility problem. We propose an insertion based framework that can achieve better results in a relatively long time period using the near future predicted demand to overcome the short-sightedness problem of the basic insertion algorithms.

In DARM, we follow the idea of searching each route and locally optimally inserting new vertex (or vertices) into a route. In our problem, there are two vertices (i.e., origin $o_{i}$ and destination $d_{i}$) to be inserted for each request $r_{i}$. We define the insertion operation as: given a vehicle $V_{j}$ with the current route $S_{V_{j}}$,  and a new request $r_{i}$, the insertion operation aims to find a new feasible route $S^{\prime}_{V_{j}}$ by inserting $o_{i}$ and $d_{i}$ into $S_{V_{j}}$ with the minimum increased cost, that is the minimum extra travel distance, while maintaining the order of vertices in $S_{V_{j}}$ unchanged in $S^{\prime}_{V_{j}}$. Specifically, for a new request $r_{i}$, the basic insertion algorithm checks every possible position to insert the origin and destination locations and return the new route such that the incremental cost is minimized. To present our cost function, we first define our distance metric, where given a graph $G$ we use our OSRM engine to pre-calculate all possible routes over our simulated city. Then, we derive the distances of the trajectories (i.e., paths) from location $a$ to location $b$ to define our graph weights. Thus, we obtain a weighted graph $G$ with realistic distance measures serving as its weights. We extend the weight notation to paths as follows:
\begin{center}
 $w(a_{1}, a_{2}, ..., a_{n}) = \sum_{i=1}^{n-1} w(a_{i}, a_{i+1})$. 
\end{center}
Thus, we define the cost associated with each new potential route/path $S^{\prime}_{V_{j}} = [r_{i}, r_{i+1}, ..., r_{k}]$ to be the $\text{cost}(V_{j}, S^{\prime}_{V_{j}}) = w(r_{i}, r_{i+1}, ... r_{k})$ resulting from this specific ordering of vertices (origin and destination locations of the $k$ requests assigned to vehicle $V_{j}$). Besides, we derive the cost of the original route to calculate the increased costs for every new route $S^{\prime}_{V_{j}}[r_{i}]$. To illustrate, assume $A_{j}$ for vehicle $V_{j}$ has only two requests $r_{x}$ and $r_{y}$, its location is $loc(V_{j})$ and its current route has $r_{x}$ already inserted as: $[loc(V_{j}), o_{x}, d_{x}]$. Then, $V_{j}$ picks $S^{\prime}_{V_{j}}$ of inserting $r_{y}$ into its current route, such that:
%\begin{equation} \label{cost}
\begin{align*}
 \text{cost}(V_{j}, S^{\prime}_{V_{j}}[r_{y}] ) = \text{min} [ &w(loc(V_{j}), o_{x}, o_{y}, d_{x}, d_{y}), \\
 &w(loc(V_{j}), o_{y}, o_{x}, d_{x}, d_{y}),\\
&w(loc(V_{j}), o_{y}, o_{x}, d_{y}, d_{x}),\\
&w(loc(V_{j}), o_{x}, o_{y}, d_{y}, d_{x}) \\
&w(loc(V_{j}), o_{x}, d_{x}, o_{y}, d_{y}) \\
&w(loc(V_{j}), o_{y}, d_{y}, o_{x}, d_{x}) ]
\end{align*}
%\end{equation}

Note that the last two optional routes complete one request before serving the other, hence they do not fit into the \textit{ride-sharing} category. However, we still take them into consideration we optimize for the fleet's overall profits and total travel distance. Also, note that these two routes will still serve both requests and thus would not affect the overall acceptance rate of our algorithm. They may just increase the customers' waiting time a little, however, we show in our results that the customers' waiting time is very reasonable. Note that if this was the first allocation made to this vehicle, then the first request will be just added to its currently empty route. Otherwise, the first request will be dealt with (like all other requests in the list) by following the insertion operation described above. Then, the cost of serving all $k$ requests in matching $A_{j}$ is in turn defined as:
\begin{equation}
 \text{cost}(V_{j}, A_{j}) = \sum_{r_{i} \in M_{j}} \text{cost}(V_{j}, S^{\prime}_{V_{j}}[r_{i}])
\end{equation}
Finally, this phase works in a distributed fashion where each vehicle minimizes its travel cost, following Algorithm \ref{insert}. This distributed procedure goes on a customer-by-customer basis as follows:
\begin{itemize}[leftmargin=*]
\item Each vehicle $V_{j}$ receives its initial matchings list $A_{j}$, and an initial price $P_{init}$ (as explained in Section \ref{init_price}) associated with each request $r_{i}$ in that list. This initial matchings list is sorted ascendingly based on proximity to vehicle $V_{j}$.
\item Then, each vehicle $V_{j}$ considers the requests in this list, in order, inserting one by one into its current route. For each request $r_{i}$, the vehicle arrives at the minimum cost  $\text{cost}(V_{j}, S^{\prime}_{V_{j}}[r_{y}] )$ associated with inserting it to its current route (as described above). 
\item Now, given the initial price associated with this request $P_{init}$ and the the new route $S^{\prime}_{V_{j}}[r_{y}]$ (which may involve detours to serve this request), the vehicle can re-calculate the pricing taking into consideration any extra distance using equation \ref{init} in Section \ref{init_price}.%, and it can also re-calculate the wating time till pickup for customer(s) associated with the request.
\item Afterwards, drivers will then modify the pricing based on the Q-values of the driver's dispatch-to location, having gained that insight using the DQN dispatch policy about which destinations can yield him/her a higher profit. The drivers weigh in on their utility function and propose a new pricing to the customer using equation \ref{car}. This procedure is explained in Section \ref{propose}.
\item Finally, the customer(s) can accept or reject based on his/her utility function as explained in Section \ref{decide}. If a customer accepts, the vehicle updates its route $S_{V_{j}}$ to be $S^{\prime}_{V_{j}}[r_{y}]$, otherwise $S_{V_{j}}$ remains unchanged. The vehicle then proceeds to the next customer and repeats the process. This rejected request will be fed back into the system to be considered in the matching process initiated  in the next timestep for other/same vehicles.
\end{itemize}

==> notations.tex <==
\begin{color}{blue} 
\begin{tabular}{ |p{5cm}||p{10cm}|  }
\hline
\textbf{Symbol} & \textbf{Description} \\
\hline
$N$   & number of vehicles    \\
\hline
${v}_{t,i}$ &   number of available vehicles at region $i$ at time slot $t$ \\
\hline
${d}_{t,i}$ & number of requests at zone $i$ at time $t$ \\
\hline
$d_{t,\widetilde{t},i}$ & the number of vehicles that are not available at time $t$ but will drop-off a passenger(s) at zone $i$ and then become available at $\widetilde{t}$ \\
\hline
${x}_{t,k}$ & current zone of vehicle $k$, available vacant seats, the time at which a passenger is picked up, and destination zone of each passenger. \\
\hline
$\varOmega_{t,n}$ &  state of vehicle $n$ at time $t$ \\
\hline
${a}_{t,n}$ & action of vehicle $n$ at time $t$ \\
\hline
$r_{t,n}$ & reward of vehicle $n$ at time $t$ \\
\hline
$\beta_i$ & weight of component $i$ in reward expression \\
\hline
$b_{t,n}$ & number of customers served by vehicle $n$ at time $t$ \\
\hline
$c_{t,n}$ & time taken by vehicle $n$ to hop or take a detour to pick up extra customers if the vehicle has available seats \\
\hline
$\delta_{t,n,\ell}$ & additional time vehicle $n$ takes because of sharing/hoping \\
\hline
$U_n$ &total number of chosen customers for pooling at vehicle $n$ \\
\hline
$\mathcal{L}_{t,n}$ & set of all customers assigned to vehicle $n$ at instant $t$ \\
\hline
$hop_{\ell,i,p}$ & $p^{th}$ hop of passenger  $\ell$ at zone $i$ \\
\hline
\end{tabular}
\end{color}
\\
\\
\rule[0.75ex]{0.60\columnwidth}{1.5pt}\\

==> route_planning.tex <==
\begin{algorithm}
	\begin{color}{blue}
	\caption{Insertion-based Route Planning}\label{route_planning_invalid}
	\begin{algorithmic}[1]
		\State \textbf{Inputs}: Vehicle $V_j$ , its current route $S_{V_j}$ , a request $r_i = (o_i , d_i)$ and weighted graph $G$ with pre-calculated trajectories using OSRM model.
		\State \textbf{Outputs}: Route $S'_{V_j}$ after insertion, with minimum $cost(V_j , S'_{V_j})$.
		\State ...
	\end{algorithmic}
	\end{color}
\end{algorithm}



